The Method of Conditional Expectations for PAPR and Cubic Metric Reduction

The OFDM waveform exhibits high fluctuation in the signal envelope which causes distortion in the nonlinear power amplifier of the transmitter. Peak-to-Average Power Ratio (PAPR) and Cubic Metric (CM) are the common metrics to quantify the phenomenon. A promising approach for PAPR or CM reduction is Sign Selection which is based on altering the signs of the data symbols. In this paper, the Method of Conditional Expectations (CE Method) is proposed to obtain a competing suboptimal solution to the Sign Selection problem. For PAPR reduction, a surrogate metric is introduced which allows for an efficient application of the CE Method. For CM reduction, the tractability of the definition of CM is exploited to this end. The algorithm is analyzed to obtain an upper bound on the worst-case reduced metric value. A noticeable characteristic is the persistent reduction capability for a wide range of subcarrier numbers. In particular, simulations show a reduction of the so-called "effective PAPR" to about 6.5 dB from 10.5 dB and 11.7 dB respectively for 64 to 1024 subcarriers. A similar steady reduction of 3 dB is observed for CM. In addition, the CE Method leads to a pruned version of Sign Selection which halves the rate loss.

==> arxiv v2 submission from v17/tikz-files/frame-double.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (13.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\foreach \x in {3,4,5}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\foreach \x in {6,7,8}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (9,1) rectangle +(0.5,-0.15);


\foreach \x in {6,7,8}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);

\foreach \x in {9,10,11}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);


\fill [draw=blue, fill=white, rounded corners=0.02cm] (12,1.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> arxiv v2 submission from v17/tikz-files/frame-single.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (7.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \xone/\y in {0/0.8, 0.5/1, 1/1.3, 1.5/1.5, 2/1.8, 2.5/2}
{
	\draw [blue,|-|] (\xone,\y) -- +(4,0);
}

\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> arxiv v2 submission from v17/tikz-files/pts-oqam-structure.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\usetikzlibrary{positioning}
%
%\input{ tikz-styles}
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}

%%%%%%%%the modulator

\node[block,minimum width=1.5cm] (filter1) {SFB};
\node[block,minimum width=1.5cm] (filter2) [below=of filter1, yshift=0.5cm] {SFB};
\node[block,minimum width=1.5cm] (filter3) [below=of filter2, yshift=0.5cm] {SFB};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (partitioning) [left of=filter1, xshift=-0.2cm, yshift=+2cm] {Partitioning};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (OQAMpre) [left of=filter1, xshift=-0.2cm, yshift=+3.8cm] {OQAM pre-preprocessing};

\node[block,minimum width=1cm, minimum height=3.7cm] (sum) [right of=filter2, xshift=4cm, yshift=0cm] {$\sum$};


\node (mul1) [summul, right of=filter1, xshift=1cm] {$\times$};
\node (mul2) [summul, right of=filter2, xshift=1.5cm] {$\times$};
\node (mul3) [summul, right of=filter3, xshift=2cm] {$\times$};

\draw [<-] (mul1) -- +(0,0.6cm) node [anchor=west]{$p_1$};
\draw [<-] (mul2) -- +(0,0.6cm) node [anchor=west]{$p_2$};
\draw [<-] (mul3) -- +(0,0.6cm) node [anchor=west]{$p_3$};

\foreach \x in {1,2,3}
	\draw [->] (filter\x) -- (mul\x);

\draw [->] (mul1.east) -- +(2.32cm,0);
\draw [->] (mul2.east) -- +(1.82cm,0);
\draw [->] (mul3.east) -- +(1.32cm,0);

\node[block,minimum width=2.4cm, minimum height=1cm] (opt) [below of=mul2, xshift=0cm, yshift=-2cm] {Optimization};

\draw [<-] (mul1) |- (opt.north);
\draw [<-] (mul2) -- (opt);
\draw [<-] (mul3) |- (opt.north);
%\draw [<-] (mul2) -- +(0cm,0);
%\draw [<-] (mul3) -- +(0cm,0);

%\foreach \x/\n in {1/0,2/1,3/N-1}
%	\draw [<-] (mul\x) -- +(0,0.5cm) node [anchor=south] {$\beta_{\n}$};

\foreach \x in {1,2,3}
{
	\draw [<-] (filter\x.west) -- +(-0.73cm,0) ;		%between SFB and partitioning
}

\draw [->] (filter1.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,0}$};  %between input and OQAM
\draw [->] (filter2.west) +(-4.5cm,0.5cm)-- +(-3.55cm,0.5cm) node [anchor=south east] {$A_{k,1}$};  %between input and OQAM
\draw [->] (filter3.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,N-1}$};  %between input and OQAM

\draw [->] (filter1.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	
\draw [->] (filter2.west) +(-2.55cm,0.5cm)-- +(-1.75cm,0.5cm) ;	%between OQAM and partitioning	
\draw [->] (filter3.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	

\node[circle, fill=black, left=of partitioning, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.3cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[circle, fill=black, left=of OQAMpre, yshift=1.9cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[block,minimum width=2cm, minimum height=1cm] (buffer) [above of=sum, xshift=-0.5cm, yshift=1.7cm] {Buffer};

\draw [->] (buffer.west) -- +(-0.3cm,0) -- +(-0.3cm,-1.2cm) -- +(1cm,-1.2cm);
\draw [->] (sum.east) +(1cm,0) |- (opt.east);
\draw [->] (sum.east) +(1cm,0) |- (buffer.east);
\draw [->] (sum.east) -- +(1.5cm,0) node [anchor=south] {$s[k]$};


	
\end{tikzpicture}
%\end{figure}
%\end{document}


==> arxiv v2 submission from v17/tikz-files/tikz-styles.tex <==
\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\tikzstyle{axis-line}=[thick, ->, >=stealth]
\tikzstyle{axis-tick}=[thin]
\tikzstyle{arrow} = [thick,->]

\tikzstyle{block}=[rectangle,black,draw, text centered, minimum height=0.7cm]
\tikzstyle{summul} = [draw, shape=circle, text centered,inner sep=0]





==> tikz-files/frame-double.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (13.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\foreach \x in {3,4,5}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\foreach \x in {6,7,8}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (9,1) rectangle +(0.5,-0.15);


\foreach \x in {6,7,8}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);

\foreach \x in {9,10,11}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,1.5) rectangle +(1,-0.15);


\fill [draw=blue, fill=white, rounded corners=0.02cm] (12,1.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/frame-single.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}
\draw [axis-line] (0,0) -- (7.5,0) node[right] {$t/T$};
\foreach \x in {0,1,2,3,4,5,6,7}
{
	\draw [axis-tick] (\x,0) -- +(0,-0.1) node[below] {\small$\x$};
}


\foreach \xone/\y in {0/0.8, 0.5/1, 1/1.3, 1.5/1.5, 2/1.8, 2.5/2}
{
	\draw [blue,|-|] (\xone,\y) -- +(4,0);
}

\foreach \x in {0,1,2}
	\fill [draw=blue, fill=blue!30!white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\foreach \x in {3,4,5}
	\fill [draw=blue, fill=white, rounded corners=0.02cm] (\x,0.5) rectangle +(1,-0.15);

\fill [draw=blue, fill=white, rounded corners=0.02cm] (6,0.5) rectangle +(0.5,-0.15);


\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}


==> tikz-files/pts-oqam-structure.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\usetikzlibrary{positioning}
%
%\input{ tikz-styles}
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}

%%%%%%%%the modulator

\node[block,minimum width=1.5cm] (filter1) {SFB};
\node[block,minimum width=1.5cm] (filter2) [below=of filter1, yshift=0.5cm] {SFB};
\node[block,minimum width=1.5cm] (filter3) [below=of filter2, yshift=0.5cm] {SFB};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (partitioning) [left of=filter1, xshift=-0.2cm, yshift=+2cm] {Partitioning};

\node[block,minimum width=3.7cm, minimum height=1cm, rotate=90] (OQAMpre) [left of=filter1, xshift=-0.2cm, yshift=+3.8cm] {OQAM pre-preprocessing};

\node[block,minimum width=1cm, minimum height=3.7cm] (sum) [right of=filter2, xshift=4cm, yshift=0cm] {$\sum$};


\node (mul1) [summul, right of=filter1, xshift=1cm] {$\times$};
\node (mul2) [summul, right of=filter2, xshift=1.5cm] {$\times$};
\node (mul3) [summul, right of=filter3, xshift=2cm] {$\times$};

\draw [<-] (mul1) -- +(0,0.6cm) node [anchor=west]{$p_1$};
\draw [<-] (mul2) -- +(0,0.6cm) node [anchor=west]{$p_2$};
\draw [<-] (mul3) -- +(0,0.6cm) node [anchor=west]{$p_3$};

\foreach \x in {1,2,3}
	\draw [->] (filter\x) -- (mul\x);

\draw [->] (mul1.east) -- +(2.32cm,0);
\draw [->] (mul2.east) -- +(1.82cm,0);
\draw [->] (mul3.east) -- +(1.32cm,0);

\node[block,minimum width=2.4cm, minimum height=1cm] (opt) [below of=mul2, xshift=0cm, yshift=-2cm] {Optimization};

\draw [<-] (mul1) |- (opt.north);
\draw [<-] (mul2) -- (opt);
\draw [<-] (mul3) |- (opt.north);
%\draw [<-] (mul2) -- +(0cm,0);
%\draw [<-] (mul3) -- +(0cm,0);

%\foreach \x/\n in {1/0,2/1,3/N-1}
%	\draw [<-] (mul\x) -- +(0,0.5cm) node [anchor=south] {$\beta_{\n}$};

\foreach \x in {1,2,3}
{
	\draw [<-] (filter\x.west) -- +(-0.73cm,0) ;		%between SFB and partitioning
}

\draw [->] (filter1.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,0}$};  %between input and OQAM
\draw [->] (filter2.west) +(-4.5cm,0.5cm)-- +(-3.55cm,0.5cm) node [anchor=south east] {$A_{k,1}$};  %between input and OQAM
\draw [->] (filter3.west) +(-4.5cm,0)-- +(-3.55cm,0) node [anchor=south east] {$A_{k,N-1}$};  %between input and OQAM

\draw [->] (filter1.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	
\draw [->] (filter2.west) +(-2.55cm,0.5cm)-- +(-1.75cm,0.5cm) ;	%between OQAM and partitioning	
\draw [->] (filter3.west) +(-2.55cm,0)-- +(-1.75cm,0) ;	%between OQAM and partitioning	

\node[circle, fill=black, left=of partitioning, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of partitioning, yshift=1.3cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[circle, fill=black, left=of OQAMpre, yshift=1.9cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.7cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};
\node[circle, fill=black, left=of OQAMpre, yshift=1.5cm, xshift=0.1cm, inner sep=0pt, minimum width=0.07cm] {};

\node[block,minimum width=2cm, minimum height=1cm] (buffer) [above of=sum, xshift=-0.5cm, yshift=1.7cm] {Buffer};

\draw [->] (buffer.west) -- +(-0.3cm,0) -- +(-0.3cm,-1.2cm) -- +(1cm,-1.2cm);
\draw [->] (sum.east) +(1cm,0) |- (opt.east);
\draw [->] (sum.east) +(1cm,0) |- (buffer.east);
\draw [->] (sum.east) -- +(1.5cm,0) node [anchor=south] {$s[k]$};


	
\end{tikzpicture}
%\end{figure}
%\end{document}

